High-energy gamma-ray and neutrino emissions from interacting supernovae based on radiation hydrodynamic simulations: a case of SN 2023ixf

Recent observations of core-collapse supernovae revealed that the existence of dense circumstellar matter (CSM) around their progenitors is ubiquitous. Interaction of supernova ejecta with such a dense CSM is a potential production sight of high-energy cosmic rays (CRs), gamma-rays, and neutrinos. We estimate the gamma-ray and neutrino signals from SN 2023ixf, a core-collapse supernova occurred in a nearby galaxy M101, which exhibits signatures of the interaction with the confined dense CSM. Using radiation-hydrodynamic simulation model calibrated by the optical and ultraviolet observations of SN 2023ixf, we find that the CRs cannot be accelerated in the early phase because the sharp velocity jump at the shock disappears due to strong radiation pressure. Roughly 4 days after the explosion, the collisionless sub-shock is formed in the CSM, which enables the CR production and leads to gamma-ray and neutrino emissions. The shock sweeps up the entire dense CSM roughly 9 days after the explosion, which ceases the high-energy radiation. Based on this scenario, we calculate the gamma-ray and neutrino signals, which have a peak around 9 days after the explosion. We can constrain the cosmic-ray production efficiency to be less than 10% by comparing our prediction to the Fermi-LAT upper limits. Future multi-messenger observations with an enlarged sample of nearby supernovae will provide a better constraint on the cosmic-ray production efficiency in the early phases of supernovae.

==> sy <==

@ARTICLE{2020PhRvD.101h3018A,
       author = {{Aharonian}, Felix and {Peron}, Giada and {Yang}, Ruizhi and {Casanova}, Sabrina and {Zanin}, Roberta},
        title = "{Probing the sea of galactic cosmic rays with Fermi-LAT}",
      journal = {\prd},
         year = 2020,
        month = apr,
       volume = {101},
       number = {8},
          eid = {083018},
        pages = {083018},
          doi = {10.1103/PhysRevD.101.083018},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020PhRvD.101h3018A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2020ApJ...901L...4B,
       author = {{Baghmanyan}, Vardan and {Peron}, Giada and {Casanova}, Sabrina and {Aharonian}, Felix and {Zanin}, Roberta},
        title = "{Evidence of Cosmic-Ray Excess from Local Giant Molecular Clouds}",
      journal = {\apjl},
     keywords = {Gamma-rays, Cosmic rays, Giant molecular clouds, 637, 329, 653, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = sep,
       volume = {901},
       number = {1},
          eid = {L4},
        pages = {L4},
          doi = {10.3847/2041-8213/abb5f8},
archivePrefix = {arXiv},
       eprint = {2009.08893},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...901L...4B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Aharonian:2018oau,
    author = "Aharonian, Felix and Yang, Ruizhi and de O\~na Wilhelmi, Emma",
    title = "{Massive Stars as Major Factories of Galactic Cosmic Rays}",
    eprint = "1804.02331",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.HE",
    doi = "10.1038/s41550-019-0724-0",
    journal = "Nature Astron.",
    volume = "3",
    number = "6",
    pages = "561--567",
    year = "2019"
}


@ARTICLE{2018ApJ...864..148K,
       author = {{Kafexhiu}, Ervin and {Romoli}, Carlo and {Taylor}, Andrew M. and {Aharonian}, Felix},
        title = "{Energetic Gamma-Ray Emission from Solar Flares}",
      journal = {\apj},
     keywords = {gamma rays: general, Sun: flares, Sun: X-rays, gamma rays, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = sep,
       volume = {864},
       number = {2},
          eid = {148},
        pages = {148},
          doi = {10.3847/1538-4357/aad801},
archivePrefix = {arXiv},
       eprint = {1803.02635},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...864..148K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2018A&A...612A..14M,
       author = {{MAGIC Collaboration} and {Ahnen}, M.~L. and {Ansoldi}, S. and
         {Antonelli}, L.~A. and {Arcaro}, C. and {Babi{\'c}}, A. and
         {Banerjee}, B. and {Bangale}, P. and {Barres de Almeida}, U. and
         {Barrio}, J.~A. and {Becerra Gonz{\'a}lez}, J. and {Bednarek}, W. and
         {Bernardini}, E. and {Berti}, A. and {Biasuzzi}, B. and {Biland}, A. and
         {Blanch}, O. and {Bonnefoy}, S. and {Bonnoli}, G. and {Borracci}, F. and
         {Carosi}, R. and {Carosi}, A. and {Chatterjee}, A. and {Colin}, P. and
         {Colombo}, E. and {Contreras}, J.~L. and {Cortina}, J. and
         {Covino}, S. and {Cumani}, P. and {da Vela}, P. and {Dazzi}, F. and
         {de Angelis}, A. and {de Lotto}, B. and {de O{\~n}a Wilhelmi}, E. and
         {di Pierro}, F. and {Doert}, M. and {Dom{\'\i}nguez}, A. and
         {Dominis Prester}, D. and {Dorner}, D. and {Doro}, M. and
         {Einecke}, S. and {Eisenacher Glawion}, D. and {Elsaesser}, D. and
         {Engelkemeier}, M. and {Fallah Ramazani}, V. and
         {Fern{\'a}ndez-Barral}, A. and {Fidalgo}, D. and {Fonseca}, M.~V. and
         {Font}, L. and {Fruck}, C. and {Galindo}, D. and
         {Garc{\'\i}a L{\'o}pez}, R.~J. and {Garczarczyk}, M. and {Gaug}, M. and
         {Giammaria}, P. and {Godinovi{\'c}}, N. and {Gora}, D. and
         {Griffiths}, S. and {Guberman}, D. and {Hadasch}, D. and {Hahn}, A. and
         {Hassan}, T. and {Hayashida}, M. and {Herrera}, J. and {Hose}, J. and
         {Hrupec}, D. and {Hughes}, G. and {Ishio}, K. and {Konno}, Y. and
         {Kubo}, H. and {Kushida}, J. and {Kuve{\v{z}}di{\'c}}, D. and
         {Lelas}, D. and {Lindfors}, E. and {Lombardi}, S. and {Longo}, F. and
         {L{\'o}pez}, M. and {L{\'o}pez-Oramas}, A. and {Majumdar}, P. and
         {Makariev}, M. and {Maneva}, G. and {Manganaro}, M. and {Mannheim}, K. and
         {Maraschi}, L. and {Mariotti}, M. and {Mart{\'\i}nez}, M. and
         {Mazin}, D. and {Menzel}, U. and {Minev}, M. and {Mirzoyan}, R. and
         {Moralejo}, A. and {Moreno}, V. and {Moretti}, E. and
         {Munar-Adrover}, P. and {Neustroev}, V. and {Niedzwiecki}, A. and
         {Nievas Rosillo}, M. and {Nilsson}, K. and {Nishijima}, K. and
         {Noda}, K. and {Nogu{\'e}s}, L. and {Paiano}, S. and {Palacio}, J. and
         {Paneque}, D. and {Paoletti}, R. and {Paredes}, J.~M. and
         {Paredes-Fortuny}, X. and {Pedaletti}, G. and {Peresano}, M. and
         {Perri}, L. and {Persic}, M. and {Prada Moroni}, P.~G. and {Prand
        ini}, E. and {Puljak}, I. and {Garcia}, J.~R. and {Reichardt}, I. and
         {Rhode}, W. and {Rib{\'o}}, M. and {Rico}, J. and {Saito}, T. and
         {Satalecka}, K. and {Schroeder}, S. and {Schweizer}, T. and
         {Shore}, S.~N. and {Sillanp{\"a}{\"a}}, A. and {Sitarek}, J. and
         {{\v{S}}nidari{\'c}}, I. and {Sobczynska}, D. and {Stamerra}, A. and
         {Strzys}, M. and {Suri{\'c}}, T. and {Takalo}, L. and {Tavecchio}, F. and
         {Temnikov}, P. and {Terzi{\'c}}, T. and {Tescaro}, D. and
         {Teshima}, M. and {Torres}, D.~F. and {Torres-Alb{\`a}}, N. and
         {Treves}, A. and {Vanzo}, G. and {Vazquez Acosta}, M. and {Vovk}, I. and
         {Ward}, J.~E. and {Will}, M. and {Wu}, M.~H. and {Zari{\'c}}, D. and
         {H.~E.~S.~S. Collaboration} and {Abdalla}, H. and {Abramowski}, A. and
         {Aharonian}, F. and {Ait Benkhali}, F. and {Akhperjanian}, A.~G. and
         {Andersson}, T. and {Ang{\"u}ner}, E.~O. and {Arakawa}, M. and
         {Arrieta}, M. and {Aubert}, P. and {Backes}, M. and {Balzer}, A. and
         {Barnard}, M. and {Becherini}, Y. and {Becker Tjus}, J. and
         {Berge}, D. and {Bernhard}, S. and {Bernl{\"o}hr}, K. and
         {Blackwell}, R. and {B{\"o}ttcher}, M. and {Boisson}, C. and
         {Bolmont}, J. and {Bordas}, P. and {Bregeon}, J. and {Brun}, F. and
         {Brun}, P. and {Bryan}, M. and {B{\"u}chele}, M. and {Bulik}, T. and
         {Capasso}, M. and {Carr}, J. and {Casanova}, S. and {Cerruti}, M. and
         {Chakraborty}, N. and {Chalme-Calvet}, R. and {Chaves}, R.~C.~G. and
         {Chen}, A. and {Chevalier}, J. and {Chr{\'e}tien}, M. and
         {Coffaro}, M. and {Colafrancesco}, S. and {Cologna}, G. and
         {Condon}, B. and {Conrad}, J. and {Cui}, Y. and {Davids}, I.~D. and
         {Decock}, J. and {Degrange}, B. and {Deil}, C. and {Devin}, J. and
         {Dewilt}, P. and {Dirson}, L. and {Djannati-Ata{\"\i}}, A. and
         {Domainko}, W. and {Donath}, A. and {Drury}, L.~O. 'c. and
         {Dutson}, K. and {Dyks}, J. and {Edwards}, T. and {Egberts}, K. and
         {Eger}, P. and {Ernenwein}, J. -P. and {Eschbach}, S. and
         {Farnier}, C. and {Fegan}, S. and {Fernandes}, M.~V. and {Fiasson}, A. and
         {Fontaine}, G. and {F{\"o}rster}, A. and {Funk}, S. and
         {F{\"u}{\ss}ling}, M. and {Gabici}, S. and {Gajdus}, M. and
         {Gallant}, Y.~A. and {Garrigoux}, T. and {Giavitto}, G. and
         {Giebels}, B. and {Glicenstein}, J.~F. and {Gottschall}, D. and
         {Goyal}, A. and {Grondin}, M. -H. and {Hahn}, J. and {Haupt}, M. and
         {Hawkes}, J. and {Heinzelmann}, G. and {Henri}, G. and {Hermann}, G. and
         {Hervet}, O. and {Hinton}, J.~A. and {Hofmann}, W. and {Hoischen}, C. and
         {Holler}, M. and {Horns}, D. and {Ivascenko}, A. and {Iwasaki}, H. and
         {Jacholkowska}, A. and {Jamrozy}, M. and {Janiak}, M. and
         {Jankowsky}, D. and {Jankowsky}, F. and {Jingo}, M. and {Jogler}, T. and
         {Jouvin}, L. and {Jung-Richardt}, I. and {Kastendieck}, M.~A. and
         {Katarzy{\'n}ski}, K. and {Katsuragawa}, M. and {Katz}, U. and
         {Kerszberg}, D. and {Khangulyan}, D. and {Kh{\'e}lifi}, B. and
         {Kieffer}, M. and {King}, J. and {Klepser}, S. and {Klochkov}, D. and
         {Klu{\'z}niak}, W. and {Kolitzus}, D. and {Komin}, Nu. and
         {Kosack}, K. and {Krakau}, S. and {Kraus}, M. and {Kr{\"u}ger}, P.~P. and
         {Laffon}, H. and {Lamanna}, G. and {Lau}, J. and {Lees}, J. -P. and
         {Lefaucheur}, J. and {Lefranc}, V. and {Lemi{\`e}re}, A. and
         {Lemoine-Goumard}, M. and {Lenain}, J. -P. and {Leser}, E. and
         {Lohse}, T. and {Lorentz}, M. and {Liu}, R. and {L{\'o}pez-Coto}, R. and
         {Lypova}, I. and {Marandon}, V. and {Marcowith}, A. and {Mariaud}, C. and
         {Marx}, R. and {Maurin}, G. and {Maxted}, N. and {Mayer}, M. and
         {Meintjes}, P.~J. and {Meyer}, M. and {Mitchell}, A.~M.~W. and
         {Moderski}, R. and {Mohamed}, M. and {Mohrmann}, L. and
         {Mor{\r{a}}}, K. and {Moulin}, E. and {Murach}, T. and {Nakashima}, S. and
         {de Naurois}, M. and {Niederwanger}, F. and {Niemiec}, J. and
         {Oakes}, L. and {O'Brien}, P. and {Odaka}, H. and {{\"O}ttl}, S. and
         {Ohm}, S. and {Ostrowski}, M. and {Oya}, I. and {Padovani}, M. and
         {Panter}, M. and {Parsons}, R.~D. and {Pekeur}, N.~W. and
         {Pelletier}, G. and {Perennes}, C. and {Petrucci}, P. -O. and
         {Peyaud}, B. and {Piel}, Q. and {Pita}, S. and {Poon}, H. and
         {Prokhorov}, D. and {Prokoph}, H. and {P{\"u}hlhofer}, G. and
         {Punch}, M. and {Quirrenbach}, A. and {Raab}, S. and {Reimer}, A. and
         {Reimer}, O. and {Renaud}, M. and {de Los Reyes}, R. and {Richter}, S. and
         {Rieger}, F. and {Romoli}, C. and {Rowell}, G. and {Rudak}, B. and
         {Rulten}, C.~B. and {Safi-Harb}, S. and {Sahakian}, V. and {Saito}, S. and
         {Salek}, D. and {Sanchez}, D.~A. and {Santangelo}, A. and {Sasaki}, M. and
         {Schlickeiser}, R. and {Sch{\"u}ssler}, F. and {Schulz}, A. and
         {Schwanke}, U. and {Schwemmer}, S. and {Seglar-Arroyo}, M. and
         {Settimo}, M. and {Seyffert}, A.~S. and {Shafi}, N. and {Shilon}, I. and
         {Simoni}, R. and {Sol}, H. and {Spanier}, F. and {Spengler}, G. and
         {Spies}, F. and {Stawarz}, {\L}. and {Steenkamp}, R. and
         {Stegmann}, C. and {Stycz}, K. and {Sushch}, I. and {Takahashi}, T. and
         {Tavernet}, J. -P. and {Tavernier}, T. and {Taylor}, A.~M. and
         {Terrier}, R. and {Tibaldo}, L. and {Tiziani}, D. and {Tluczykont}, M. and
         {Trichard}, C. and {Tsuji}, N. and {Tuffs}, R. and {Uchiyama}, Y. and
         {van der Walt}, D.~J. and {van Eldik}, C. and {van Rensburg}, C. and
         {van Soelen}, B. and {Vasileiadis}, G. and {Veh}, J. and {Venter}, C. and
         {Viana}, A. and {Vincent}, P. and {Vink}, J. and {Voisin}, F. and
         {V{\"o}lk}, H.~J. and {Vuillaume}, T. and {Wadiasingh}, Z. and
         {Wagner}, S.~J. and {Wagner}, P. and {Wagner}, R.~M. and {White}, R. and
         {Wierzcholska}, A. and {Willmann}, P. and {W{\"o}rnlein}, A. and
         {Wouters}, D. and {Yang}, R. and {Zabalza}, V. and {Zaborov}, D. and
         {Zacharias}, M. and {Zanin}, R. and {Zdziarski}, A.~A. and {Zech}, A. and
         {Zefi}, F. and {Ziegler}, A. and {Zywucka}, N.},
        title = "{Constraints on particle acceleration in SS433/W50 from MAGIC and H.E.S.S. observations}",
      journal = {\aap},
     keywords = {gamma rays: general, stars: black holes, X-rays: binaries, ISM: jets and outflows, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2018",
        month = "Apr",
       volume = {612},
          eid = {A14},
        pages = {A14},
          doi = {10.1051/0004-6361/201731169},
archivePrefix = {arXiv},
       eprint = {1707.03658},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...612A..14M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{AYO18a,
   author = {{Aharonian}, F. and {Yang}, R. and {de O{\~n}a Wilhelmi}, E.
	},
    title = "{Massive Stars as Major Factories of Galactic Cosmic Rays}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1804.02331},
 primaryClass = "astro-ph.HE",
 keywords = {Astrophysics - High Energy Astrophysical Phenomena},
     year = 2018,
    month = apr,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180402331A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{HESS17a,
   author = {{Abdalla}, H. and {Abramowski}, A. and {Aharonian}, F. and {Ait Benkhali}, F. and 
	{Ang{\"u}ner}, E.~O. and {Arakawa}, M. and {Arrieta}, M. and 
	{Aubert}, P. and {Backes}, M. and {Balzer}, A. and et al.},
    title = "{TeV Gamma-Ray Observations of the Binary Neutron Star Merger GW170817 with H.E.S.S.}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1710.05862},
 primaryClass = "astro-ph.HE",
 keywords = {gamma-ray burst: individual: GRB 170817A, gamma rays: general, gravitational waves},
     year = 2017,
    month = dec,
   volume = 850,
      eid = {L22},
    pages = {L22},
      doi = {10.3847/2041-8213/aa97d2},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...850L..22A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016Natur.531..476H,
       author = {{HESS Collaboration} and {Abramowski}, A. and {Aharonian}, F. and {Benkhali}, F. Ait and {Akhperjanian}, A.~G. and {Ang{\"u}ner}, E.~O. and {Backes}, M. and {Balzer}, A. and {Becherini}, Y. and {Tjus}, J. Becker and {Berge}, D. and {Bernhard}, S. and {Bernl{\"o}hr}, K. and {Birsin}, E. and {Blackwell}, R. and {B{\"o}ttcher}, M. and {Boisson}, C. and {Bolmont}, J. and {Bordas}, P. and {Bregeon}, J. and {Brun}, F. and {Brun}, P. and {Bryan}, M. and {Bulik}, T. and {Carr}, J. and {Casanova}, S. and {Chakraborty}, N. and {Chalme-Calvet}, R. and {Chaves}, R.~C.~G. and {Chen}, A. and {Chr{\'e}tien}, M. and {Colafrancesco}, S. and {Cologna}, G. and {Conrad}, J. and {Couturier}, C. and {Cui}, Y. and {Davids}, I.~D. and {Degrange}, B. and {Deil}, C. and {Dewilt}, P. and {Djannati-Ata{\"\i}}, A. and {Domainko}, W. and {Donath}, A. and {Drury}, L. O'C. and {Dubus}, G. and {Dutson}, K. and {Dyks}, J. and {Dyrda}, M. and {Edwards}, T. and {Egberts}, K. and {Eger}, P. and {Ernenwein}, J. -P. and {Espigat}, P. and {Farnier}, C. and {Fegan}, S. and {Feinstein}, F. and {Fernandes}, M.~V. and {Fernandez}, D. and {Fiasson}, A. and {Fontaine}, G. and {F{\"o}rster}, A. and {F{\"u}{\ss}ling}, M. and {Gabici}, S. and {Gajdus}, M. and {Gallant}, Y.~A. and {Garrigoux}, T. and {Giavitto}, G. and {Giebels}, B. and {Glicenstein}, J.~F. and {Gottschall}, D. and {Goyal}, A. and {Grondin}, M. -H. and {Grudzi{\'n}ska}, M. and {Hadasch}, D. and {H{\"a}ffner}, S. and {Hahn}, J. and {Hawkes}, J. and {Heinzelmann}, G. and {Henri}, G. and {Hermann}, G. and {Hervet}, O. and {Hillert}, A. and {Hinton}, J.~A. and {Hofmann}, W. and {Hofverberg}, P. and {Hoischen}, C. and {Holler}, M. and {Horns}, D. and {Ivascenko}, A. and {Jacholkowska}, A. and {Jamrozy}, M. and {Janiak}, M. and {Jankowsky}, F. and {Jung-Richardt}, I. and {Kastendieck}, M.~A. and {Katarzy{\'n}ski}, K. and {Katz}, U. and {Kerszberg}, D. and {Kh{\'e}lifi}, B. and {Kieffer}, M. and {Klepser}, S. and {Klochkov}, D. and {Klu{\'z}niak}, W. and {Kolitzus}, D. and {Komin}, Nu. and {Kosack}, K. and {Krakau}, S. and {Krayzel}, F. and {Kr{\"u}ger}, P.~P. and {Laffon}, H. and {Lamanna}, G. and {Lau}, J. and {Lefaucheur}, J. and {Lefranc}, V. and {Lemi{\'e}re}, A. and {Lemoine-Goumard}, M. and {Lenain}, J. -P. and {Lohse}, T. and {Lopatin}, A. and {Lu}, C. -C. and {Lui}, R. and {Marandon}, V. and {Marcowith}, A. and {Mariaud}, C. and {Marx}, R. and {Maurin}, G. and {Maxted}, N. and {Mayer}, M. and {Meintjes}, P.~J. and {Menzler}, U. and {Meyer}, M. and {Mitchell}, A.~M.~W. and {Moderski}, R. and {Mohamed}, M. and {Mor{\r{a}}}, K. and {Moulin}, E. and {Murach}, T. and {de Naurois}, M. and {Niemiec}, J. and {Oakes}, L. and {Odaka}, H. and {{\"O}ttl}, S. and {Ohm}, S. and {Opitz}, B. and {Ostrowski}, M. and {Oya}, I. and {Panter}, M. and {Parsons}, R.~D. and {Arribas}, M. Paz and {Pekeur}, N.~W. and {Pelletier}, G. and {Petrucci}, P. -O. and {Peyaud}, B. and {Pita}, S. and {Poon}, H. and {Prokoph}, H. and {P{\"u}hlhofer}, G. and {Punch}, M. and {Quirrenbach}, A. and {Raab}, S. and {Reichardt}, I. and {Reimer}, A. and {Reimer}, O. and {Renaud}, M. and {de Los Reyes}, R. and {Rieger}, F. and {Romoli}, C. and {Rosier-Lees}, S. and {Rowell}, G. and {Rudak}, B. and {Rulten}, C.~B. and {Sahakian}, V. and {Salek}, D. and {Sanchez}, D.~A. and {Santangelo}, A. and {Sasaki}, M. and {Schlickeiser}, R. and {Sch{\"u}ssler}, F. and {Schulz}, A. and {Schwanke}, U. and {Schwemmer}, S. and {Seyffert}, A.~S. and {Simoni}, R. and {Sol}, H. and {Spanier}, F. and {Spengler}, G. and {Spies}, F. and {Stawarz}, {\L}. and {Steenkamp}, R. and {Stegmann}, C. and {Stinzing}, F. and {Stycz}, K. and {Sushch}, I. and {Tavernet}, J. -P. and {Tavernier}, T. and {Taylor}, A.~M. and {Terrier}, R. and {Tluczykont}, M. and {Trichard}, C. and {Tuffs}, R. and {Valerius}, K. and {van der Walt}, J. and {van Eldik}, C. and {van Soelen}, B. and {Vasileiadis}, G. and {Veh}, J. and {Venter}, C. and {Viana}, A. and {Vincent}, P. and {Vink}, J. and {Voisin}, F. and {V{\"o}lk}, H.~J. and {Vuillaume}, T. and {Wagner}, S.~J. and {Wagner}, P. and {Wagner}, R.~M. and {Weidinger}, M. and {Weitzel}, Q. and {White}, R. and {Wierzcholska}, A. and {Willmann}, P. and {W{\"o}rnlein}, A. and {Wouters}, D. and {Yang}, R. and {Zabalza}, V. and {Zaborov}, D. and {Zacharias}, M. and {Zdziarski}, A.~A. and {Zech}, A. and {Zefi}, F. and {{\.Z}ywucka}, N.},
        title = "{Acceleration of petaelectronvolt protons in the Galactic Centre}",
      journal = {\nat},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = mar,
       volume = {531},
       number = {7595},
        pages = {476-479},
          doi = {10.1038/nature17147},
archivePrefix = {arXiv},
       eprint = {1603.07730},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016Natur.531..476H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{KM3NeT16a,
   author = {{Adri{\'a}n-Mart{\'{\i}}nez}, S. and {Ageron}, M. and {Aharonian}, F. and 
	{Aiello}, S. and {Albert}, A. and {Ameli}, F. and {Anassontzis}, E. and 
	{Andre}, M. and {Androulakis}, G. and {Anghinolfi}, M. and et al.},
    title = "{Letter of intent for KM3NeT 2.0}",
  journal = {Journal of Physics G Nuclear Physics},
archivePrefix = "arXiv",
   eprint = {1601.07459},
 primaryClass = "astro-ph.IM",
     year = 2016,
    month = aug,
   volume = 43,
   number = 8,
      eid = {084001},
    pages = {084001},
      doi = {10.1088/0954-3899/43/8/084001},
   adsurl = {http://adsabs.harvard.edu/abs/2016JPhG...43h4001A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2015ApJ...807L...8B,
       author = {{Bordas}, P. and {Yang}, R. and {Kafexhiu}, E. and {Aharonian}, F.},
        title = "{Detection of Persistent Gamma-Ray Emission Toward SS433/W50}",
      journal = {\apjl},
     keywords = {binaries: general, gamma rays: general, ISM: jets and outflows, stars: individual: SS433, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2015",
        month = "Jul",
       volume = {807},
       number = {1},
          eid = {L8},
        pages = {L8},
          doi = {10.1088/2041-8205/807/1/L8},
archivePrefix = {arXiv},
       eprint = {1411.7413},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...807L...8B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2014PhRvD..89h3004L,
       author = {{Liu}, Ruo-Yu and {Wang}, Xiang-Yu and {Inoue}, Susumu and {Crocker},
        Roland and {Aharonian}, Felix},
        title = "{Diffuse PeV neutrinos from EeV cosmic ray sources: Semirelativistic hypernova remnants in star-forming galaxies}",
      journal = {\prd},
     keywords = {95.85.Ry, 98.58.Mj, 98.70.Sa, Neutrino muon pion and other elementary particles, cosmic rays, Supernova remnants, Cosmic rays, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = Apr,
       volume = {89},
          eid = {083004},
        pages = {083004},
          doi = {10.1103/PhysRevD.89.083004},
archivePrefix = {arXiv},
       eprint = {1310.1263},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2014PhRvD..89h3004L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2014PhRvD..90l3014K,
   author = {{Kafexhiu}, E. and {Aharonian}, F. and {Taylor}, A.~M. and {Vila}, G.~S.
	},
    title = "{Parametrization of gamma-ray production cross sections for p p interactions in a broad proton energy range from the kinematic threshold to PeV energies}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1406.7369},
 primaryClass = "astro-ph.HE",
 keywords = {Nucleon-nucleon interactions, Inclusive production with identified hadrons, Cosmic-ray interactions},
     year = 2014,
    month = dec,
   volume = 90,
   number = 12,
      eid = {123014},
    pages = {123014},
      doi = {10.1103/PhysRevD.90.123014},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..90l3014K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Aha13a,
   author = {{Aharonian}, F.~A.},
    title = "{Gamma rays from supernova remnants}",
  journal = {Astroparticle Physics},
     year = 2013,
    month = mar,
   volume = 43,
    pages = {71-80},
      doi = {10.1016/j.astropartphys.2012.08.007},
   adsurl = {http://adsabs.harvard.edu/abs/2013APh....43...71A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{sah+13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...770L...6S},
	Archiveprefix = {arXiv},
	Author = {{Sahakyan}, N. and {Yang}, R. and {Aharonian}, F.~A. and {Rieger}, F.~M.},
	Doi = {10.1088/2041-8205/770/1/L6},
	Eid = {L6},
	Eprint = {1302.7173},
	Journal = {\apjl},
	Keywords = {galaxies: active, galaxies: individual: Cen A},
	Month = jun,
	Pages = {L6},
	Primaryclass = {astro-ph.HE},
	Title = {{Evidence for a Second Component in the High-energy Core Emission from Centaurus A?}},
	Volume = 770,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/770/1/L6}}


@ARTICLE{2012ApJ...746..151A,
       author = {{Abramowski}, A. and {Acero}, F. and {Aharonian}, F. and
         {Akhperjanian}, A.~G. and {Anton}, G. and {Balzer}, A. and
         {Barnacka}, A. and {Barres de Almeida}, U. and {Becherini}, Y. and
         {Becker}, J. and {Behera}, B. and {Bernl{\"o}hr}, K. and {Birsin}, E. and
         {Biteau}, J. and {Bochow}, A. and {Boisson}, C. and {Bolmont}, J. and
         {Bordas}, P. and {Brucker}, J. and {Brun}, F. and {Brun}, P. and
         {Bulik}, T. and {B{\"u}sching}, I. and {Carrigan}, S. and
         {Casanova}, S. and {Cerruti}, M. and {Chadwick}, P.~M. and
         {Charbonnier}, A. and {Chaves}, R.~C.~G. and {Cheesebrough}, A. and
         {Clapson}, A.~C. and {Coignet}, G. and {Cologna}, G. and {Conrad}, J. and
         {Dalton}, M. and {Daniel}, M.~K. and {Davids}, I.~D. and
         {Degrange}, B. and {Deil}, C. and {Dickinson}, H.~J. and
         {Djannati-Ata{\"\i}}, A. and {Domainko}, W. and {Drury}, L. O'C. and
         {Dubus}, G. and {Dutson}, K. and {Dyks}, J. and {Dyrda}, M. and
         {Egberts}, K. and {Eger}, P. and {Espigat}, P. and {Fallon}, L. and
         {Farnier}, C. and {Fegan}, S. and {Feinstein}, F. and {Fernand
        es}, M.~V. and {Fiasson}, A. and {Fontaine}, G. and {F{\"o}rster}, A. and
         {F{\"u}{\ss}ling}, M. and {Gallant}, Y.~A. and {Gast}, H. and
         {G{\'e}rard}, L. and {Gerbig}, D. and {Giebels}, B. and
         {Glicenstein}, J.~F. and {Gl{\"u}ck}, B. and {Goret}, P. and
         {G{\"o}ring}, D. and {H{\"a}ffner}, S. and {Hague}, J.~D. and
         {Hampf}, D. and {Hauser}, M. and {Heinz}, S. and {Heinzelmann}, G. and
         {Henri}, G. and {Hermann}, G. and {Hinton}, J.~A. and {Hoffmann}, A. and
         {Hofmann}, W. and {Hofverberg}, P. and {Holler}, M. and {Horns}, D. and
         {Jacholkowska}, A. and {de Jager}, O.~C. and {Jahn}, C. and
         {Jamrozy}, M. and {Jung}, I. and {Kastendieck}, M.~A. and
         {Katarzy{\'n}ski}, K. and {Katz}, U. and {Kaufmann}, S. and
         {Keogh}, D. and {Khangulyan}, D. and {Kh{\'e}lifi}, B. and
         {Klochkov}, D. and {Klu{\'z}niak}, W. and {Kneiske}, T. and
         {Komin}, Nu. and {Kosack}, K. and {Kossakowski}, R. and {Laffon}, H. and
         {Lamanna}, G. and {Lennarz}, D. and {Lohse}, T. and {Lopatin}, A. and
         {Lu}, C. -C. and {Marandon}, V. and {Marcowith}, A. and {Masbou}, J. and
         {Maurin}, D. and {Maxted}, N. and {Mayer}, M. and {McComb}, T.~J.~L. and
         {Medina}, M.~C. and {M{\'e}hault}, J. and {Moderski}, R. and
         {Moulin}, E. and {Naumann}, C.~L. and {Naumann-Godo}, M. and
         {de Naurois}, M. and {Nedbal}, D. and {Nekrassov}, D. and {Nguyen}, N. and
         {Nicholas}, B. and {Niemiec}, J. and {Nolan}, S.~J. and {Ohm}, S. and
         {de O{\~n}a Wilhelmi}, E. and {Opitz}, B. and {Ostrowski}, M. and
         {Oya}, I. and {Panter}, M. and {Paz Arribas}, M. and {Pedaletti}, G. and
         {Pelletier}, G. and {Petrucci}, P. -O. and {Pita}, S. and
         {P{\"u}hlhofer}, G. and {Punch}, M. and {Quirrenbach}, A. and
         {Raue}, M. and {Rayner}, S.~M. and {Reimer}, A. and {Reimer}, O. and
         {Renaud}, M. and {de los Reyes}, R. and {Rieger}, F. and {Ripken}, J. and
         {Rob}, L. and {Rosier-Lees}, S. and {Rowell}, G. and {Rudak}, B. and
         {Rulten}, C.~B. and {Ruppel}, J. and {Sahakian}, V. and
         {Sanchez}, D.~A. and {Santangelo}, A. and {Schlickeiser}, R. and
         {Sch{\"o}ck}, F.~M. and {Schulz}, A. and {Schwanke}, U. and
         {Schwarzburg}, S. and {Schwemmer}, S. and {Sheidaei}, F. and
         {Skilton}, J.~L. and {Sol}, H. and {Spengler}, G. and {Stawarz}, {\L}. and
         {Steenkamp}, R. and {Stegmann}, C. and {Stinzing}, F. and {Stycz}, K. and
         {Sushch}, I. and {Szostek}, A. and {Tavernet}, J. -P. and
         {Terrier}, R. and {Tluczykont}, M. and {Valerius}, K. and
         {van Eldik}, C. and {Vasileiadis}, G. and {Venter}, C. and
         {Vialle}, J.~P. and {Viana}, A. and {Vincent}, P. and
         {V{\"o}lk}, H.~J. and {Volpe}, F. and {Vorobiov}, S. and {Vorster}, M. and
         {Wagner}, S.~J. and {Ward}, M. and {White}, R. and {Wierzcholska}, A. and
         {Zacharias}, M. and {Zajczyk}, A. and {Zdziarski}, A.~A. and
         {Zech}, A. and {Zechlin}, H. -S. and {H.~E.~S.~S. Collaboration} and
         {Aleksi{\'c}}, J. and {Antonelli}, L.~A. and {Antoranz}, P. and
         {Backes}, M. and {Barrio}, J.~A. and {Bastieri}, D. and
         {Becerra Gonz{\'a}lez}, J. and {Bednarek}, W. and {Berdyugin}, A. and
         {Berger}, K. and {Bernardini}, E. and {Biland}, A. and {Blanch}, O. and
         {Bock}, R.~K. and {Boller}, A. and {Bonnoli}, G. and
         {Borla Tridon}, D. and {Braun}, I. and {Bretz}, T. and
         {Ca{\~n}ellas}, A. and {Carmona}, E. and {Carosi}, A. and {Colin}, P. and
         {Colombo}, E. and {Contreras}, J.~L. and {Cortina}, J. and
         {Cossio}, L. and {Covino}, S. and {Dazzi}, F. and {De Angelis}, A. and
         {De Cea del Pozo}, E. and {De Lotto}, B. and {Delgado Mendez}, C. and
         {Diago Ortega}, A. and {Doert}, M. and {Dom{\'\i}nguez}, A. and
         {Dominis Prester}, D. and {Dorner}, D. and {Doro}, M. and
         {Elsaesser}, D. and {Ferenc}, D. and {Fonseca}, M.~V. and {Font}, L. and
         {Fruck}, C. and {Garc{\'\i}a L{\'o}pez}, R.~J. and {Garczarczyk}, M. and
         {Garrido}, D. and {Giavitto}, G. and {Godinovi{\'c}}, N. and
         {Hadasch}, D. and {H{\"a}fner}, D. and {Herrero}, A. and {Hildebrand
        }, D. and {H{\"o}hne-M{\"o}nch}, D. and {Hose}, J. and {Hrupec}, D. and
         {Huber}, B. and {Jogler}, T. and {Klepser}, S. and
         {Kr{\"a}henb{\"u}hl}, T. and {Krause}, J. and {La Barbera}, A. and
         {Lelas}, D. and {Leonardo}, E. and {Lindfors}, E. and {Lombardi}, S. and
         {L{\'o}pez}, M. and {Lorenz}, E. and {Makariev}, M. and {Maneva}, G. and
         {Mankuzhiyil}, N. and {Mannheim}, K. and {Maraschi}, L. and
         {Mariotti}, M. and {Mart{\'\i}nez}, M. and {Mazin}, D. and
         {Meucci}, M. and {Miranda}, J.~M. and {Mirzoyan}, R. and
         {Miyamoto}, H. and {Mold{\'o}n}, J. and {Moralejo}, A. and {Munar}, P. and
         {Nieto}, D. and {Nilsson}, K. and {Orito}, R. and {Oya}, I. and
         {Paneque}, D. and {Paoletti}, R. and {Pardo}, S. and {Paredes}, J.~M. and
         {Partini}, S. and {Pasanen}, M. and {Pauss}, F. and
         {Perez-Torres}, M.~A. and {Persic}, M. and {Peruzzo}, L. and
         {Pilia}, M. and {Pochon}, J. and {Prada}, F. and {Prada Moroni}, P.~G. and
         {Prandini}, E. and {Puljak}, I. and {Reichardt}, I. and {Reinthal}, R. and
         {Rhode}, W. and {Rib{\'o}}, M. and {Rico}, J. and {R{\"u}gamer}, S. and
         {Saggion}, A. and {Saito}, K. and {Saito}, T.~Y. and {Salvati}, M. and
         {Satalecka}, K. and {Scalzotto}, V. and {Scapin}, V. and {Schultz}, C. and
         {Schweizer}, T. and {Shayduk}, M. and {Shore}, S.~N. and
         {Sillanp{\"a}{\"a}}, A. and {Sitarek}, J. and {Sobczynska}, D. and
         {Spanier}, F. and {Spiro}, S. and {Stamerra}, A. and {Steinke}, B. and
         {Storz}, J. and {Strah}, N. and {Suri{\'c}}, T. and {Takalo}, L. and
         {Takami}, H. and {Tavecchio}, F. and {Temnikov}, P. and
         {Terzi{\'c}}, T. and {Tescaro}, D. and {Teshima}, M. and {Thom}, M. and
         {Tibolla}, O. and {Torres}, D.~F. and {Treves}, A. and {Vankov}, H. and
         {Vogler}, P. and {Wagner}, R.~M. and {Weitzel}, Q. and {Zabalza}, V. and
         {Zandanel}, F. and {Zanin}, R. and {MAGIC Collaboration} and
         {Arlen}, T. and {Aune}, T. and {Beilicke}, M. and {Benbow}, W. and
         {Bouvier}, A. and {Bradbury}, S.~M. and {Buckley}, J.~H. and
         {Bugaev}, V. and {Byrum}, K. and {Cannon}, A. and {Cesarini}, A. and
         {Ciupik}, L. and {Connolly}, M.~P. and {Cui}, W. and {Dickherber}, R. and
         {Duke}, C. and {Errando}, M. and {Falcone}, A. and {Finley}, J.~P. and
         {Finnegan}, G. and {Fortson}, L. and {Furniss}, A. and {Galante}, N. and
         {Gall}, D. and {Godambe}, S. and {Griffin}, S. and {Grube}, J. and
         {Gyuk}, G. and {Hanna}, D. and {Holder}, J. and {Huan}, H. and
         {Hui}, C.~M. and {Kaaret}, P. and {Karlsson}, N. and {Kertzman}, M. and
         {Khassen}, Y. and {Kieda}, D. and {Krawczynski}, H. and
         {Krennrich}, F. and {Lang}, M.~J. and {LeBohec}, S. and {Maier}, G. and
         {McArthur}, S. and {McCann}, A. and {Moriarty}, P. and {Mukherjee}, R. and
         {Nu{\~n}ez}, P.~D. and {Ong}, R.~A. and {Orr}, M. and {Otte}, A.~N. and
         {Park}, N. and {Perkins}, J.~S. and {Pichel}, A. and {Pohl}, M. and
         {Prokoph}, H. and {Ragan}, K. and {Reyes}, L.~C. and {Reynolds}, P.~T. and
         {Roache}, E. and {Rose}, H.~J. and {Ruppel}, J. and {Schroedter}, M. and
         {Sembroski}, G.~H. and {{\c{S}}ent{\"u}rk}, G.~D. and
         {Telezhinsky}, I. and {Te{\v{s}}i{\'c}}, G. and {Theiling}, M. and
         {Thibadeau}, S. and {Varlotta}, A. and {Vassiliev}, V.~V. and
         {Vivier}, M. and {Wakely}, S.~P. and {Weekes}, T.~C. and
         {Williams}, D.~A. and {Zitzer}, B. and {VERITAS Collaboration} and
         {Barres de Almeida}, U. and {Cara}, M. and {Casadio}, C. and
         {Cheung}, C.~C. and {McConville}, W. and {Davies}, F. and {Doi}, A. and
         {Giovannini}, G. and {Giroletti}, M. and {Hada}, K. and {Hardee}, P. and
         {Harris}, D.~E. and {Junor}, W. and {Kino}, M. and {Lee}, N.~P. and
         {Ly}, C. and {Madrid}, J. and {Massaro}, F. and {Mundell}, C.~G. and
         {Nagai}, H. and {Perlman}, E.~S. and {Steele}, I.~A. and
         {Walker}, R.~C. and {Wood}, D.~L.},
        title = "{The 2010 Very High Energy {\ensuremath{\gamma}}-Ray Flare and 10 Years of Multi-wavelength Observations of M 87}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: individual: M 87, galaxies: jets, galaxies: nuclei, gamma rays: galaxies, radiation mechanisms: non-thermal, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2012,
        month = feb,
       volume = {746},
       number = {2},
          eid = {151},
        pages = {151},
          doi = {10.1088/0004-637X/746/2/151},
archivePrefix = {arXiv},
       eprint = {1111.5341},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...746..151A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{che+11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...726...60C},
	Archiveprefix = {arXiv},
	Author = {{Chernyakova}, M. and {Malyshev}, D. and {Aharonian}, F.~A. and {Crocker}, R.~M. and {Jones}, D.~I.},
	Doi = {10.1088/0004-637X/726/2/60},
	Eid = {60},
	Eprint = {1009.2630},
	Journal = {\apj},
	Keywords = {cosmic rays, diffusion, Galaxy: center, gamma rays: general},
	Month = jan,
	Pages = {60},
	Primaryclass = {astro-ph.HE},
	Title = {{The High-energy, Arcminute-scale Galactic Center Gamma-ray Source}},
	Volume = 726,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/726/2/60}}


@ARTICLE{2010ApJ...724.1517B,
   author = {{Barkov}, M.~V. and {Aharonian}, F.~A. and {Bosch-Ramon}, V.
	},
    title = "{Gamma-ray Flares from Red Giant/Jet Interactions in Active Galactic Nuclei}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1005.5252},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, galaxies: jets, gamma rays: galaxies, hydrodynamics, radiation mechanisms: non-thermal, stars: flare},
     year = 2010,
    month = dec,
   volume = 724,
    pages = {1517-1523},
      doi = {10.1088/0004-637X/724/2/1517},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...724.1517B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{hess09gc,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...503..817A},
	Archiveprefix = {arXiv},
	Author = {{Aharonian}, F. and {Akhperjanian}, A.~G. and {Anton}, G. and {Barres de Almeida}, U. and {Bazer-Bachi}, A.~R. and {Becherini}, Y. and {Behera}, B. and {Bernl{\"o}hr}, K. and {Boisson}, C. and {Bochow}, A. and {Borrel}, V. and {Braun}, I. and {Brion}, E. and {Brucker}, J. and {Brun}, P. and {B{\"u}hler}, R. and {Bulik}, T. and {B{\"u}sching}, I. and {Boutelier}, T. and {Chadwick}, P.~M. and {Charbonnier}, A. and {Chaves}, R.~C.~G. and {Cheesebrough}, A. and {Chounet}, L.-M. and {Clapson}, A.~C. and {Coignet}, G. and {Dalton}, M. and {Daniel}, M.~K. and {Davids}, I.~D. and {Degrange}, B. and {Deil}, C. and {Dickinson}, H.~J. and {Djannati-Ata{\"\i}}, A. and {Domainko}, W. and {O'C.~Drury}, L. and {Dubois}, F. and {Dubus}, G. and {Dyks}, J. and {Dyrda}, M. and {Egberts}, K. and {Emmanoulopoulos}, D. and {Espigat}, P. and {Farnier}, C. and {Feinstein}, F. and {Fiasson}, A. and {F{\"o}rster}, A. and {Fontaine}, G. and {F{\"u}{\ss}ling}, M. and {Gabici}, S. and {Gallant}, Y.~A. and {G{\'e}rard}, L. and {Giebels}, B. and {Glicenstein}, J.~F. and {Gl{\"u}ck}, B. and {Goret}, P. and {Hauser}, D. and {Hauser}, M. and {Heinz}, S. and {Heinzelmann}, G. and {Henri}, G. and {Hermann}, G. and {Hinton}, J.~A. and {Hoffmann}, A. and {Hofmann}, W. and {Holleran}, M. and {Hoppe}, S. and {Horns}, D. and {Jacholkowska}, A. and {de Jager}, O.~C. and {Jung}, I. and {Katarzy{\'n}ski}, K. and {Katz}, U. and {Kaufmann}, S. and {Kendziorra}, E. and {Kerschhaggl}, M. and {Khangulyan}, D. and {Kh{\'e}lifi}, B. and {Keogh}, D. and {Komin}, N. and {Kosack}, K. and {Lamanna}, G. and {Lenain}, J.-P. and {Lohse}, T. and {Marandon}, V. and {Martin}, J.~M. and {Martineau-Huynh}, O. and {Marcowith}, A. and {Maurin}, D. and {McComb}, T.~J.~L. and {Medina}, M.~C. and {Moderski}, R. and {Moulin}, E. and {Naumann-Godo}, M. and {de Naurois}, M. and {Nedbal}, D. and {Nekrassov}, D. and {Niemiec}, J. and {Nolan}, S.~J. and {Ohm}, S. and {Olive}, J.-F. and {de O{\~n}a Wilhelmi}, E. and {Orford}, K.~J. and {Ostrowski}, M. and {Panter}, M. and {Paz Arribas}, M. and {Pedaletti}, G. and {Pelletier}, G. and {Petrucci}, P.-O. and {Pita}, S. and {P{\"u}hlhofer}, G. and {Punch}, M. and {Quirrenbach}, A. and {Raubenheimer}, B.~C. and {Raue}, M. and {Rayner}, S.~M. and {Renaud}, M. and {Rieger}, F. and {Ripken}, J. and {Rob}, L. and {Rolland}, L. and {Rosier-Lees}, S. and {Rowell}, G. and {Rudak}, B. and {Rulten}, C.~B. and {Ruppel}, J. and {Sahakian}, V. and {Santangelo}, A. and {Schlickeiser}, R. and {Sch{\"o}ck}, F.~M. and {Schr{\"o}der}, R. and {Schwanke}, U. and {Schwarzburg}, S. and {Schwemmer}, S. and {Shalchi}, A. and {Skilton}, J.~L. and {Sol}, H. and {Spangler}, D. and {Stawarz}, {\L}. and {Steenkamp}, R. and {Stegmann}, C. and {Superina}, G. and {Szostek}, A. and {Tam}, P.~H. and {Tavernet}, J.-P. and {Terrier}, R. and {Tibolla}, O. and {van Eldik}, C. and {Vasileiadis}, G. and {Venter}, C. and {Venter}, L. and {Vialle}, J.~P. and {Vincent}, P. and {Vivier}, M. and {V{\"o}lk}, H.~J. and {Volpe}, F. and {Wagner}, S.~J. and {Ward}, M. and {Zdziarski}, A.~A. and {Zech}, A.},
	Doi = {10.1051/0004-6361/200811569},
	Eprint = {0906.1247},
	Journal = {\aap},
	Keywords = {Galaxy: center, gamma rays: observations, methods: data analysis},
	Month = sep,
	Pages = {817-825},
	Primaryclass = {astro-ph.GA},
	Title = {{Spectrum and variability of the Galactic center VHE {$\gamma$}-ray source HESS J1745-290}},
	Volume = 503,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200811569}}


@article{hess09cenA,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...695L..40A},
	Archiveprefix = {arXiv},
	Author = {{Aharonian}, F. and {Akhperjanian}, A.~G. and {Anton}, G. and {de Almeida}, U.~B. and {Bazer-Bachi}, A.~R. and {Becherini}, Y. and {Behera}, B. and {Benbow}, W. and {Bernl{\"o}hr}, K. and {Boisson}, C. and {Bochow}, A. and {Borrel}, V. and {Brion}, E. and {Brucker}, J. and {Brun}, P. and {B{\"u}hler}, R. and {Bulik}, T. and {B{\"u}sching}, I. and {Boutelier}, T. and {Chadwick}, P.~M. and {Charbonnier}, A. and {Chaves}, R.~C.~G. and {Cheesebrough}, A. and {Chounet}, L.-M. and {Clapson}, A.~C. and {Coignet}, G. and {Dalton}, M. and {Daniel}, M.~K. and {Davids}, I.~D. and {Degrange}, B. and {Deil}, C. and {Dickinson}, H.~J. and {Djannati-Ata{\"\i}}, A. and {Domainko}, W. and {Drury}, L.~O. and {Dubois}, F. and {Dubus}, G. and {Dyks}, J. and {Dyrda}, M. and {Egberts}, K. and {Emmanoulopoulos}, D. and {Espigat}, P. and {Farnier}, C. and {Feinstein}, F. and {Fiasson}, A. and {F{\"o}rster}, A. and {Fontaine}, G. and {F{\"u}{\ss}ling}, M. and {Gabici}, S. and {Gallant}, Y.~A. and {G{\'e}rard}, L. and {Giebels}, B. and {Glicenstein}, J.-F. and {Gl{\"u}ck}, B. and {Goret}, P. and {G{\"o}hring}, D. and {Hauser}, D. and {Hauser}, M. and {Heinz}, S. and {Heinzelmann}, G. and {Henri}, G. and {Hermann}, G. and {Hinton}, J.~A. and {Hoffmann}, A. and {Hofmann}, W. and {Holleran}, M. and {Hoppe}, S. and {Horns}, D. and {Jacholkowska}, A. and {de Jager}, O.~C. and {Jahn}, C. and {Jung}, I. and {Katarzy{\'n}ski}, K. and {Katz}, U. and {Kaufmann}, S. and {Kendziorra}, E. and {Kerschhaggl}, M. and {Khangulyan}, D. and {Kh{\'e}lifi}, B. and {Keogh}, D. and {Klu{\'z}niak}, W. and {Kneiske}, T. and {Komin}, N. and {Kosack}, K. and {Lamanna}, G. and {Latham}, I.~J. and {Lenain}, J.-P. and {Lohse}, T. and {Marandon}, V. and {Martin}, J.~M. and {Martineau-Huynh}, O. and {Marcowith}, A. and {Maurin}, D. and {McComb}, T.~J.~L. and {Medina}, M.~C. and {Moderski}, R. and {Moulin}, E. and {Naumann-Godo}, M. and {de Naurois}, M. and {Nedbal}, D. and {Nekrassov}, D. and {Niemiec}, J. and {Nolan}, S.~J. and {Ohm}, S. and {Olive}, J.-F. and {de O{\~n}a Wilhelmi}, E. and {Orford}, K.~J. and {Ostrowski}, M. and {Panter}, M. and {Arribas}, M.~P. and {Pedaletti}, G. and {Pelletier}, G. and {Petrucci}, P.-O. and {Pita}, S. and {P{\"u}hlhofer}, G. and {Punch}, M. and {Quirrenbach}, A. and {Raubenheimer}, B.~C. and {Raue}, M. and {Rayner}, S.~M. and {Renaud}, M. and {Rieger}, F. and {Ripken}, J. and {Rob}, L. and {Rosier-Lees}, S. and {Rowell}, G. and {Rudak}, B. and {Rulten}, C.~B. and {Ruppel}, J. and {Sahakian}, V. and {Santangelo}, A. and {Schlickeiser}, R. and {Sch{\"o}ck}, F.~M. and {Schr{\"o}der}, R. and {Schwanke}, U. and {Schwarzburg}, S. and {Schwemmer}, S. and {Shalchi}, A. and {Sikora}, M. and {Skilton}, J.~L. and {Sol}, H. and {Spangler}, D. and {Stawarz}, {\L}. and {Steenkamp}, R. and {Stegmann}, C. and {Superina}, G. and {Szostek}, A. and {Tam}, P.~H. and {Tavernet}, J.-P. and {Terrier}, R. and {Tibolla}, O. and {Tluczykont}, M. and {van Eldik}, C. and {Vasileiadis}, G. and {Venter}, C. and {Venter}, L. and {Vialle}, J.~P. and {Vincent}, P. and {Vink}, J. and {Vivier}, M. and {V{\"o}lk}, H.~J. and {Volpe}, F. and {Wagner}, S.~J. and {Ward}, M. and {Zdziarski}, A.~A. and {Zech}, A.},
	Doi = {10.1088/0004-637X/695/1/L40},
	Eprint = {0903.1582},
	Journal = {\apjl},
	Keywords = {galaxies: active, galaxies: individual: Cen A, gamma rays: observations},
	Month = apr,
	Pages = {L40-L44},
	Primaryclass = {astro-ph.CO},
	Title = {{Discovery of Very High Energy {$\gamma$}-Ray Emission from Centaurus a with H.E.S.S.}},
	Volume = 695,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/695/1/L40}}


@ARTICLE{KA08a,
   author = {{Kelner}, S.~R. and {Aharonian}, F.~A.},
    title = "{Energy spectra of gamma rays, electrons, and neutrinos produced at interactions of relativistic protons with low energy radiation}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {0803.0688},
 keywords = {Specific calculations, Decays of pi mesons, Photon and charged-lepton interactions with hadrons, Inclusive production with identified leptons photons or other nonhadronic particles},
     year = 2008,
    month = aug,
   volume = 78,
   number = 3,
      eid = {034013},
    pages = {034013},
      doi = {10.1103/PhysRevD.78.034013},
   adsurl = {http://adsabs.harvard.edu/abs/2008PhRvD..78c4013K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{hess06gc,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006PhRvL..97v1102A},
	Author = {{Aharonian}, F. and {Akhperjanian}, A.~G. and {Bazer-Bachi}, A.~R. and {Beilicke}, M. and {Benbow}, W. and {Berge}, D. and {Bernl{\"o}hr}, K. and {Boisson}, C. and {Bolz}, O. and {Borrel}, V. and {Braun}, I. and {Breitling}, F. and {Brown}, A.~M. and {B{\"u}hler}, R. and {B{\"u}sching}, I. and {Carrigan}, S. and {Chadwick}, P.~M. and {Chounet}, L.-M. and {Cornils}, R. and {Costamante}, L. and {Degrange}, B. and {Dickinson}, H.~J. and {Djannati-Ata{\"\i}}, A. and {Drury}, L.~O.~'. and {Dubus}, G. and {Egberts}, K. and {Emmanoulopoulos}, D. and {Espigat}, P. and {Feinstein}, F. and {Ferrero}, E. and {Fiasson}, A. and {Fontaine}, G. and {Funk}, S. and {Funk}, S. and {Gallant}, Y.~A. and {Giebels}, B. and {Glicenstein}, J.~F. and {Goret}, P. and {Hadjichristidis}, C. and {Hauser}, D. and {Hauser}, M. and {Heinzelmann}, G. and {Henri}, G. and {Hermann}, G. and {Hinton}, J.~A. and {Hofmann}, W. and {Holleran}, M. and {Horns}, D. and {Jacholkowska}, A. and {de Jager}, O.~C. and {Kh{\'e}lifi}, B. and {Komin}, N. and {Konopelko}, A. and {Kosack}, K. and {Latham}, I.~J. and {Le Gallou}, R. and {Lemi{\`e}re}, A. and {Lemoine-Goumard}, M. and {Lohse}, T. and {Martin}, J.~M. and {Martineau-Huynh}, O. and {Marcowith}, A. and {Masterson}, C. and {McComb}, T.~J.~L. and {de Naurois}, M. and {Nedbal}, D. and {Nolan}, S.~J. and {Noutsos}, A. and {Orford}, K.~J. and {Osborne}, J.~L. and {Ouchrif}, M. and {Panter}, M. and {Pelletier}, G. and {Pita}, S. and {P{\"u}hlhofer}, G. and {Punch}, M. and {Raubenheimer}, B.~C. and {Raue}, M. and {Rayner}, S.~M. and {Reimer}, A. and {Reimer}, O. and {Ripken}, J. and {Rob}, L. and {Rolland}, L. and {Rowell}, G. and {Sahakian}, V. and {Saug{\'e}}, L. and {Schlenker}, S. and {Schlickeiser}, R. and {Schwanke}, U. and {Sol}, H. and {Spangler}, D. and {Spanier}, F. and {Steenkamp}, R. and {Stegmann}, C. and {Superina}, G. and {Tavernet}, J.-P. and {Terrier}, R. and {Th{\'e}oret}, C.~G. and {Tluczykont}, M. and {van Eldik}, C. and {Vasileiadis}, G. and {Venter}, C. and {Vincent}, P. and {V{\"o}lk}, H.~J. and {Wagner}, S.~J. and {Ward}, M.},
	Doi = {10.1103/PhysRevLett.97.221102},
	Eid = {221102},
	Eprint = {astro-ph/0610509},
	Journal = {Physical Review Letters},
	Month = dec,
	Number = 22,
	Pages = {221102},
	Title = {{HESS Observations of the Galactic Center Region and Their Possible Dark Matter Interpretation}},
	Volume = 97,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevLett.97.221102}}


@article{hess06m87,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006Sci...314.1424A},
	Author = {{Aharonian}, F. and {Akhperjanian}, A.~G. and {Bazer-Bachi}, A.~R. and {Beilicke}, M. and {Benbow}, W. and {Berge}, D. and {Bernl{\"o}hr}, K. and {Boisson}, C. and {Bolz}, O. and {Borrel}, V. and {Braun}, I. and {Brown}, A.~M. and {B{\"u}hler}, R. and {B{\"u}sching}, I. and {Carrigan}, S. and {Chadwick}, P.~M. and {Chounet}, L.-M. and {Coignet}, G. and {Cornils}, R. and {Costamante}, L. and {Degrange}, B. and {Dickinson}, H.~J. and {Djannati-Ata{\"\i}}, A. and {Drury}, L.~O. and {Dubus}, G. and {Egberts}, K. and {Emmanoulopoulos}, D. and {Espigat}, P. and {Feinstein}, F. and {Ferrero}, E. and {Fiasson}, A. and {Fontaine}, G. and {Funk}, S. and {Funk}, S. and {F{\"u}{\ss}ling}, M. and {Gallant}, Y.~A. and {Giebels}, B. and {Glicenstein}, J.~F. and {Goret}, P. and {Hadjichristidis}, C. and {Hauser}, D. and {Hauser}, M. and {Heinzelmann}, G. and {Henri}, G. and {Hermann}, G. and {Hinton}, J.~A. and {Hoffmann}, A. and {Hofmann}, W. and {Holleran}, M. and {Hoppe}, S. and {Horns}, D. and {Jacholkowska}, A. and {de Jager}, O.~C. and {Kendziorra}, E. and {Kerschhaggl}, M. and {Kh{\'e}lifi}, B. and {Komin}, N. and {Konopelko}, A. and {Kosack}, K. and {Lamanna}, G. and {Latham}, I.~J. and {Le Gallou}, R. and {Lemi{\`e}re}, A. and {Lemoine-Goumard}, M. and {Lenain}, J.-P. and {Lohse}, T. and {Martin}, J.~M. and {Martineau-Huynh}, O. and {Marcowith}, A. and {Masterson}, C. and {Maurin}, G. and {McComb}, T.~J.~L. and {Moulin}, E. and {de Naurois}, M. and {Nedbal}, D. and {Nolan}, S.~J. and {Noutsos}, A. and {Orford}, K.~J. and {Osborne}, J.~L. and {Ouchrif}, M. and {Panter}, M. and {Pelletier}, G. and {Pita}, S. and {P{\"u}hlhofer}, G. and {Punch}, M. and {Ranchon}, S. and {Raubenheimer}, B.~C. and {Raue}, M. and {Rayner}, S.~M. and {Reimer}, A. and {Ripken}, J. and {Rob}, L. and {Rolland}, L. and {Rosier-Lees}, S. and {Rowell}, G. and {Sahakian}, V. and {Santangelo}, A. and {Saug{\'e}}, L. and {Schlenker}, S. and {Schlickeiser}, R. and {Schr{\"o}der}, R. and {Schwanke}, U. and {Schwarzburg}, S. and {Schwemmer}, S. and {Shalchi}, A. and {Sol}, H. and {Spangler}, D. and {Spanier}, F. and {Steenkamp}, R. and {Stegmann}, C. and {Superina}, G. and {Tam}, P.~H. and {Tavernet}, J.-P. and {Terrier}, R. and {Tluczykont}, M. and {van Eldik}, C. and {Vasileiadis}, G. and {Venter}, C. and {Vialle}, J.~P. and {Vincent}, P. and {V{\"o}lk}, H.~J. and {Wagner}, S.~J. and {Ward}, M.},
	Doi = {10.1126/science.1134408},
	Eprint = {astro-ph/0612016},
	Journal = {Science},
	Month = dec,
	Pages = {1424-1427},
	Title = {{Fast Variability of Tera-Electron Volt {$\gamma$} Rays from the Radio Galaxy M87}},
	Volume = 314,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.1134408}}


@article{kab06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006PhRvD..74c4018K},
	Author = {{Kelner}, S.~R. and {Aharonian}, F.~A. and {Bugayov}, V.~V.},
	Doi = {10.1103/PhysRevD.74.034018},
	Eid = {034018},
	Eprint = {astro-ph/0606058},
	Journal = {\prd},
	Keywords = {Nucleon-nucleon interactions, Decays of pi mesons, Total and inclusive cross sections, Leptons},
	Month = aug,
	Number = 3,
	Pages = {034018},
	Title = {{Energy spectra of gamma rays, electrons, and neutrinos produced at proton-proton interactions in the very high energy regime}},
	Volume = 74,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevD.74.034018}}


@article{an05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...619..306A},
	Author = {{Aharonian}, F. and {Neronov}, A.},
	Doi = {10.1086/426426},
	Eprint = {astro-ph/0408303},
	Journal = {\apj},
	Keywords = {Acceleration of Particles, Black Hole Physics, Galaxy: Nucleus, Gamma Rays: Theory},
	Month = jan,
	Pages = {306-313},
	Title = {{High-Energy Gamma Rays from the Massive Black Hole in the Galactic Center}},
	Volume = 619,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/426426}}


@ARTICLE{2000A&A...362..937A,
       author = {{Aharonian}, F.~A. and {Atoyan}, A.~M.},
        title = "{Broad-band diffuse gamma ray emission of the galactic disk}",
      journal = {\aap},
     keywords = {RADIATION MECHANISMS: NON-THERMAL, ISM: COSMIC RAYS, GALAXY: GENERAL, GAMMA RAYS: THEORY, Astrophysics},
         year = 2000,
        month = oct,
       volume = {362},
        pages = {937-952},
archivePrefix = {arXiv},
       eprint = {astro-ph/0009009},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...362..937A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1997ApJ...487L...9C,
       author = {{Coppi}, Paolo S. and {Aharonian}, Felix A.},
        title = "{Constraints on the Very High Energy Emissivity of the Universe from the Diffuse GeV Gamma-Ray Background}",
      journal = {\apj},
     keywords = {COSMOLOGY: DIFFUSE RADIATION, GAMMA RAYS: THEORY, RADIATIVE TRANSFER, GALAXIES: ACTIVE, Cosmology: Diffuse Radiation, Galaxies: Active, Gamma Rays: Theory, Radiative Transfer, Astrophysics},
         year = "1997",
        month = "Sep",
       volume = {487},
       number = {1},
        pages = {L9-L12},
          doi = {10.1086/310883},
archivePrefix = {arXiv},
       eprint = {astro-ph/9610176},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...487L...9C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
